Learning Deep Sensorimotor Policies for Vision-based Autonomous Drone Racing

Autonomous drones can operate in remote and unstructured environments, enabling various real-world applications. However, the lack of effective vision-based algorithms has been a stumbling block to achieving this goal. Existing systems often require hand-engineered components for state estimation, planning, and control. Such a sequential design involves laborious tuning, human heuristics, and compounding delays and errors. This paper tackles the vision-based autonomous-drone-racing problem by learning deep sensorimotor policies. We use contrastive learning to extract robust feature representations from the input images and leverage a two-stage learning-by-cheating framework for training a neural network policy. The resulting policy directly infers control commands with feature representations learned from raw images, forgoing the need for globally-consistent state estimation, trajectory planning, and handcrafted control design. Our experimental results indicate that our vision-based policy can achieve the same level of racing performance as the state-based policy while being robust against different visual disturbances and distractors. We believe this work serves as a stepping-stone toward developing intelligent vision-based autonomous systems that control the drone purely from image inputs, like human pilots.

==> sections/05limitation.tex <==
\section{Limitation}
% A fundamental research question in drone control is that is it possible to control the drone directly with images, like professional human pilots. 
% % 
% Our vision-based end-to-end control system still relies on some parts of the drone state, such as the orientation.  
% % 
% From a classical control perspective, this is due to the requirement of having observability of the continuous system. 

% \TODO{Add limitations of transfer into real world experiments}
%

%
% Sim to real transfer techniques such as transfer learning still need to be applied for robust performance in real world.


==> tables/ablation_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htp]
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{} & \multirow{2}{*}{}    & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Contrastive\\ Learning\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Random\\ Convolution\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Random\\ Cutout-color\end{tabular}} & \multicolumn{3}{c}{Success Rate} \\ \cline{6-8} 
& & & &  & Circle    & Figure8   & SplitS   \\ \hline
\multirow{3}{*}{Brightness Change} & \multirow{3}{*}{0.5} 
& \textcolor{blue}{\cmark}  & \textcolor{blue}{\cmark}  & \textcolor{red}{\xmark} & \textbf{1.0} & \textbf{0.8} & \textbf{1.0} \\
&  & \textcolor{red}{\xmark} & \textcolor{blue}{\cmark} & \textcolor{red}{\xmark} & 0.0 & 0.0 & 0.0 \\
&  & \textcolor{red}{\xmark} & \textcolor{red}{\xmark}  & \textcolor{red}{\xmark} & 0.0 & 0.0 & 0.0 \\ \hline
\multirow{3}{*}{Hue Change} & \multirow{3}{*}{0.5} 
& \textcolor{blue}{\cmark} & \textcolor{blue}{\cmark} & \textcolor{red}{\xmark}  & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
& & \textcolor{red}{\xmark} & \textcolor{blue}{\cmark} & \textcolor{red}{\xmark} & 1.0 & 0.0 & 0.0 \\
& & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{red}{\xmark}  & 0.0 & 0.0 & 0.0 \\ \hline
\multirow{3}{*}{Blue Boxes} & \multirow{3}{*}{60}  
& \textcolor{blue}{\cmark} & \textcolor{red}{\xmark} & \textcolor{blue}{\cmark} & \textbf{1.0} & \textbf{1.0} &  \textbf{0.9} \\
& & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{blue}{\cmark} & 0.0 & 0.0 & 0.0 \\
& & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & 0.0 & 0.0 & 0.0 \\ \hline
\multirow{3}{*}{Random Objects} & \multirow{3}{*}{60} 
&  \textcolor{blue}{\cmark} & \textcolor{red}{\xmark} & \textcolor{blue}{\cmark}   & \textbf{1.0} & \textbf{0.6} & \textbf{1.0}  \\
& & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{blue}{\cmark} & 0.0 & 0.0 & 0.0 \\
& & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} & \textcolor{red}{\xmark}  & 0.0 & 0.0 & 0.0 \\ \hline
\end{tabular}
\vspace{0.5mm}
\caption{Ablation study of contrastive learning and data augmentation}
\label{tab:ablation}
\vspace{-4mm}
\end{table}

==> tables/ablation_distractor.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{cc|ccc|ccc|ccc}
\multicolumn{2}{c|}{\multirow{2}{*}{}}           & \multicolumn{3}{c|}{SplitS}            & \multicolumn{3}{c|}{Figure8}           & \multicolumn{3}{c}{Circle}             \\ \cline{3-11} 
\multicolumn{2}{c|}{}                            & Original   & Overlay    & Naive Cutout & Original   & Overlay    & Naive Cutout & Original   & Overlay    & Naive Cutout \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{Blue}}  & 10 & 1.00(0.00) & 0.00(0.00) & 0.20(0.42)   & 0.50(0.53) & 1.00(0.00) & 1.00(0.00)   & 1.00(0.00) & 1.00(0.00) & 1.00(0.00)   \\
\multicolumn{1}{c|}{}                       & 20 & 0.00(0.00) & 0.00(0.00) & 0.00(0.00)   & 0.00(0.00) & 0.90(0.32) & 1.00(0.00)   & 0.00(0.00) & 1.00(0.00) & 1.00(0.00)   \\
\multicolumn{1}{c|}{}                       & 30 & 0.00(0.00) & 0.00(0.00) & 0.00(0.00)   & 0.00(0.00) & 0.80(0.42) & 1.00(0.00)   & 0.00(0.00) & 1.00(0.00) & 0.10(0.32)   \\
\multicolumn{1}{c|}{}                       & 40 & 0.00(0.00) & 0.00(0.00) & 0.00(0.00)   & 0.00(0.00) & 0.80(0.42) & 0.60(0.52)   & 0.00(0.00) & 1.00(0.00) & 0.00(0.00)   \\
\multicolumn{1}{c|}{}                       & 50 & 0.00(0.00) & 0.00(0.00) & 0.00(0.00)   & 0.00(0.00) & 0.60(0.52) & 0.50(0.53)   & 0.00(0.00) & 1.00(0.00) & 0.00(0.00)   \\
\multicolumn{1}{c|}{}                       & 60 & 0.00(0.00) & 0.00(0.00) & 0.00(0.00)   & 0.00(0.00) & 0.40(0.52) & 0.40(0.52)   & 0.00(0.00) & 1.00(0.00) & 0.00(0.00)   \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{Green}} & 10 & 0.00(0.00) & 0.00(0.00) & 1.00(0.00)   & 0.00(0.00) & 0.10(0.32) & 1.00(0.00)   & 0.00(0.00) & 1.00(0.00) & 0.00(0.00)   \\
\multicolumn{1}{c|}{}                       & 20 & 0.00(0.00) & 0.00(0.00) & 1.00(0.00)   & 0.00(0.00) & 0.00(0.00) & 1.00(0.00)   & 0.00(0.00) & 0.00(0.00) & 0.00(0.00)   \\
\multicolumn{1}{c|}{}                       & 30 & 0.00(0.00) & 0.00(0.00) & 1.00(0.00)   & 0.00(0.00) & 0.00(0.00) & 1.00(0.00)   & 0.00(0.00) & 0.00(0.00) & 0.00(0.00)   \\
\multicolumn{1}{c|}{}                       & 40 & 0.00(0.00) & 0.00(0.00) & 0.00(0.00)   & 0.00(0.00) & 0.00(0.00) & 0.40(0.52)   & 0.00(0.00) & 0.00(0.00) & 0.00(0.00)   \\
\multicolumn{1}{c|}{}                       & 50 & 0.00(0.00) & 0.00(0.00) & 0.00(0.00)   & 0.00(0.00) & 0.00(0.00) & 0.10(0.32)   & 0.00(0.00) & 0.00(0.00) & 0.00(0.00)   \\
\multicolumn{1}{c|}{}                       & 60 & 0.00(0.00) & 0.00(0.00) & 0.00(0.00)   & 0.00(0.00) & 0.00(0.00) & 0.10(0.32)   & 0.00(0.00) & 0.00(0.00) & 0.00(0.00)  
\end{tabular}
\end{table}

==> tables/ablation_reb_data_aug.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htp]
\centering
\begin{tabular}{clccccc}
\hline
\multirow{2}{*}{}                  & \multirow{2}{*}{}    & Random                   & Random                   & \multicolumn{3}{c}{Success rate} \\ \cline{5-7} 
                                   &                      & Convolution              & Cutout-color             & Cricle    & Figure8   & SplitS   \\ \hline
\multirow{2}{*}{Brightness Change} & \multirow{2}{*}{0.5} & \textcolor{blue}{\cmark} & \textcolor{red}{\xmark}  & 1.0       & 0.8       & 1.0      \\
                                   &                      & \textcolor{red}{\xmark}  & \textcolor{red}{\xmark}  & 0.0       & 0.0       & 0.0      \\ \hline
\multirow{2}{*}{Hue Change}        & \multirow{2}{*}{0.5} & \textcolor{blue}{\cmark} & \textcolor{red}{\xmark}  & 1.0       & 1.0       & 1.0      \\
                                   &                      & \textcolor{red}{\xmark}  & \textcolor{red}{\xmark}  & 0.0       & 0.0       & 0.0      \\ \hline
\multirow{2}{*}{Blue Boxes}        & \multirow{2}{*}{60}  & \textcolor{red}{\xmark}  & \textcolor{blue}{\cmark} & 1.0       & 1.0       & 0.9      \\
                                   &                      & \textcolor{red}{\xmark}  & \textcolor{red}{\xmark}  & 0.0       & 0.0       & 0.0      \\ \hline
\multirow{2}{*}{Random Objects}    & \multirow{2}{*}{60}  & \textcolor{red}{\xmark}  & \textcolor{blue}{\cmark} & 1.0       & 0.6       & 1.0      \\
                                   &                      & \textcolor{red}{\xmark}  & \textcolor{red}{\xmark}  & 0.0       & 0.0       & 0.0      \\ \hline
\end{tabular}
\vspace{0.5mm}
\caption{Ablation study of data augmentation}
\label{tab:ablation_reb_data_aug}
\vspace{-4mm}
\end{table}

==> tables/ablation_reb_latent.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htp]
\centering
\begin{tabular}{cccc}
\hline
\multirow{2}{*}{Track}  & \multirow{2}{*}{Latent Loss} & \multicolumn{2}{c}{Success rate} \\ \cline{3-4} 
                        &                              & Before 3000\nth   & Before 6000\nth  \\ \hline
\multirow{2}{*}{SplitS} & \textcolor{blue}{\cmark}     & 1.0             & 1.0            \\
                        & \textcolor{red}{\xmark}      & 0.5             & 1.0            \\ \hline
\end{tabular}
\vspace{0.5mm}
\caption{Ablation study of latent space loss}
\label{tab:ablation_reb_latent}
\vspace{-4mm}
\end{table}

==> tables/ablation_reb_mem.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htp]
\centering
\begin{tabular}{ccc}
\hline
Track                   & Network Architecture & Success Rate \\ \hline
\multirow{3}{*}{SplitS} & TCN                  & 1.0         \\
                        & RNN                  & 0.9         \\
                        & MLP                  & 0.3         \\ \hline
\end{tabular}
\vspace{0.5mm}
\caption{Ablation study of memory-based networks}
\label{tab:ablation_reb_mem}
\vspace{-4mm}
\end{table}

==> tables/ablation_reb_norm.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htp]
\centering
\begin{tabular}{ccc}
\hline
Track                   & Image Feature Normalization & Success rate \\ \hline
\multirow{2}{*}{SplitS} & \textcolor{blue}{\cmark}    & 1.0          \\
                        & \textcolor{red}{\xmark}     & 0.9         \\ \hline
\end{tabular}
\vspace{0.5mm}
\caption{Ablation study of image feature normalization}
\label{tab:ablation_reb_norm}
\vspace{-4mm}
\end{table}

==> tables/ablation_reb_state.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htbp]
\centering
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{Track}  & \multicolumn{4}{c}{Drone States}                                                                                                                      & \multirow{2}{*}{Success Rate} \\ \cline{2-5}
                        & \multicolumn{1}{l}{Orientation} & \multicolumn{1}{l}{Linear Velocity} & \multicolumn{1}{l}{Linear Acceleration} & \multicolumn{1}{l}{Previous Action} &                               \\ \hline
\multirow{6}{*}{SplitS} & \textcolor{blue}{\cmark}        & \textcolor{blue}{\cmark}            & \textcolor{blue}{\cmark}                & \textcolor{blue}{\cmark}            & 1.0                           \\
                        & \textcolor{red}{\xmark}         & \textcolor{blue}{\cmark}            & \textcolor{blue}{\cmark}                & \textcolor{blue}{\cmark}            & 1.0                           \\
                        & \textcolor{blue}{\cmark}        & \textcolor{red}{\xmark}             & \textcolor{blue}{\cmark}                & \textcolor{blue}{\cmark}            & 0.2                          \\
                        & \textcolor{blue}{\cmark}        & \textcolor{blue}{\cmark}            & \textcolor{red}{\xmark}                 & \textcolor{blue}{\cmark}            & 0.7                           \\
                        & \textcolor{blue}{\cmark}        & \textcolor{blue}{\cmark}            & \textcolor{blue}{\cmark}                & \textcolor{red}{\xmark}             & 0.7                           \\
                        & \textcolor{red}{\xmark}         & \textcolor{red}{\xmark}             & \textcolor{red}{\xmark}                 & \textcolor{red}{\xmark}             & 0.0                           \\ \bottomrule 
\end{tabular}
\vspace{0.5mm}
\caption{Ablation study of additional drone states}
\label{tab:ablation_reb_state}
\vspace{-4mm}
\end{table}

==> tables/baseline_time_optimal.tex <==
\begin{table}[htp]
\centering
\begin{tabular}{cccc}
\hline
& Circle (s) & Figure8 (s) & SplitS (s) \\ \hline
Time Optimal Trajectory\cite{Foehn2021science} & 4.68 & 6.26 & 7.93 \\
Vision-based Policy (\textbf{Ours}) & 4.95 & 6.76 & 8.58    \\ \hline
\end{tabular}
\vspace{0.5em} 
\caption{Benchmark comparison between our vision-based policy and time-optimal planning~\cite{Foehn2021science}.
Our vision-based policy achieved near-time-optimal flight in all three different tracks. 
}
\label{tab:baseline_time_optimal}
\vspace{-5mm}
\end{table}

==> tables/benchmark.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{l|lll}
\toprule
               & Circle & Figure8 & SplitS \\ \midrule
VIO            & 0.2    & 0.2     & 0.2    \\
Teacher Policy & 1.0    & 1.0     & 1.0    \\
Student Policy & 1.0    & 1.0     & 1.0    \\ \bottomrule
\end{tabular}
\caption{}
\label{}
\end{table}

==> tables/drone_config.tex <==
\begin{table}[!htb] 
   \centering 
   \footnotesize 
   % {
   \renewcommand{\tabcolsep}{4.4pt} 
   \renewcommand{\arraystretch}{0.8} 
   \begin{tabular}{c|cc|cc}
     \toprule 
  & Variable & Value & Variable & Value \\%[-0.2em] %& Variable & Value \\
   \midrule 
   \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Drone}}} & Weight [\SI{}{\kg}] & 0.752 & Arm Length [\SI{}{\meter}] & 0.15 \\
   & $f_{min}$ [\SI{}{\newton}] & 0 & $f_{max}$ [\SI{}{\newton}] & 3.61 \\
   & $\text{diag}(J)$ [\SI{}{\gram\metre\squared}] & $[2.5,2.1,4.3]$ & $\kappa$ [-] & 0.022 \\
   & $w_{max}$ [\SI{}{\radian\per\second}] & 8 & $c_{f}$ & \num{1.563e-6} \\
   \midrule 
   \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{PPO}}} & Action network & [128, 128] & Value network & [512, 512] \\
   & GAE $\lambda$ & 0.95 & Discount factor $\gamma$ & 0.98 \\
   & Value function coefficient & 0.5 & Entropy Coefficient & 0.0 \\
   & Maximum gradient norm & 0.5 & Learning rate & \num{3e-5} \\
   & Clipping range & 0.2 & Batch size & 25000 \\
   & Total training iterations & 2000 & Samples per iteration & 250000 \\
   \midrule 
   \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{IL}}} 
   & Policy network & [128, 64, 32] & Policy activation & leaky ReLU \\
   & TCN network & [512, 512] & TCN kernel size & 3 \\
   & TCN dropout & 0.1 & Latent loss coefficient $\lambda$ & 0.5 \\
   & Learning rate & \num{3e-4} & Batch size & 2048 \\
   & History length & 16 & Skipping frames & 2 \\
   & Number of replay buffers & 7 & & \\
   \bottomrule 
   \end{tabular}  
   \vspace{0.5em} 
   \caption{Hyperparameters.}  
   \label{tab: hyperparameters}
\end{table} 

==> tables/raw_perform.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{l|ccccccccc}
\toprule
            & & \multicolumn{2}{c}{Cirle} & & \multicolumn{2}{c}{Figure8} & & \multicolumn{2}{c}{SplitS} \\
             \cline{3-4} \cline{6-7} \cline{9-10} 
             && Teacher     & Student     && Teacher      & Student      && Teacher      & Student     \\ \midrule
Lap Time(s)  & & 4.97(0.01)        & 4.95(0.01)        & & 6.84(0.05)         & 6.76(0.01)         & & 8.74(0.01)         & 8.58(0.01)        \\
Success Rate & & 1.00        & 1.00        & & 1.00         & 1.00         & & 1.00         & 1.00        \\ 
\bottomrule
\end{tabular}
\caption{}
\label{}
\end{table}


==> tables/transfer_perform_distract.tex <==
% \begin{table}[htbp]
% \centering
% \begin{tabular}{ll|lll}
% \toprule
% \multicolumn{2}{l|}{}                            & SplitS     & Figure8    & Circle     \\ \midrule
% \multicolumn{1}{l|}{\multirow{6}{*}{Blue}}  & 10 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 20 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 30 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 40 & 0.9 & 0.9 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 50 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 60 & 0.9 & 1.0 & 1.0 \\ \midrule
% \multicolumn{1}{l|}{\multirow{6}{*}{Random}} & 10 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 20 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 30 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 40 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 50 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 60 & 1.0 & 0.6 & 1.0 \\ \bottomrule
% \end{tabular}
% \caption{Success rate when increasing the number of blue and random distractors.}
% \label{tab:distractor}
% \end{table}

\begin{table}[htbp]
\centering
\begin{tabular}{cccccccc}
\toprule
 \multirow{2}{*}{\textit{\#(Distractors)}} & \multicolumn{3}{c}{\textbf{Blue Boxes}} && \multicolumn{3}{c}{\textbf{Random Obstacles}} \\
 \cline{2-4} \cline{6-8}
  & SplitS     & Figure8    & Circle && SplitS     & Figure8    & Circle \\
 \midrule
 \textit{10} & 1.0 & 1.0 & 1.0 && 1.0 & 1.0 & 1.0 \\
% \textit{20} & 1.0 & 1.0 & 1.0 && 1.0 & 1.0 & 1.0 \\
% \textit{30} & 1.0 & 1.0 & 1.0 && 1.0 & 1.0 & 1.0 \\
% \textit{40} & 0.9 & 0.9 & 1.0 && 1.0 & 1.0 & 1.0 \\
% \textit{50} & 1.0 & 1.0 & 1.0 && 1.0 & 1.0 & 1.0 \\
 \textit{60} & 0.9 & 1.0 & 1.0 && 1.0 & 0.6 & 1.0 \\
 \bottomrule
% \multicolumn{2}{l|}{}                            & SplitS     & Figure8    & Circle     \\ \midrule
% \multicolumn{1}{l|}{\multirow{6}{*}{Blue}}  & 10 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 20 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 30 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 40 & 0.9 & 0.9 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 50 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 60 & 0.9 & 1.0 & 1.0 \\ \midrule
% \multicolumn{1}{l|}{\multirow{6}{*}{Random}} & 10 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 20 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 30 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 40 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 50 & 1.0 & 1.0 & 1.0 \\
% \multicolumn{1}{l|}{}                       & 60 & 1.0 & 0.6 & 1.0 \\ \bottomrule
\end{tabular}
\caption{Success rate when increasing the number of blue and random distractors.}
\label{tab:distractor-new}
\end{table}

==> tables/transfer_perform_incr_distract.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{l|cccllll}
\hline
Number of Distractors & 8   & 15   & 30  & 40  & 60   & 80  & 100 \\ \hline
Success Rate40        & 1.0 & 0.85 & 0.9 & 1.0 & 0.95 & 0.6 & 0.3 \\ \hline
\end{tabular}
\end{table}
